A Survey of Recent Scalability Improvements for Semidefinite Programming with Applications in Machine Learning, Control, and Robotics

Historically, scalability has been a major challenge to the successful application of semidefinite programming in fields such as machine learning, control, and robotics. In this paper, we survey recent approaches for addressing this challenge including (i) approaches for exploiting structure (e.g., sparsity and symmetry) in a problem, (ii) approaches that produce low-rank approximate solutions to semidefinite programs, (iii) more scalable algorithms that rely on augmented Lagrangian techniques and the alternating direction method of multipliers, and (iv) approaches that trade off scalability with conservatism (e.g., by approximating semidefinite programs with linear and second-order cone programs). For each class of approaches we provide a high-level exposition, an entry-point to the corresponding literature, and examples drawn from machine learning, control, or robotics. We also present a list of software packages that implement many of the techniques discussed in the paper. Our hope is that this paper will serve as a gateway to the rich and exciting literature on scalable semidefinite programming for both theorists and practitioners.

==> sections/low_rank_night.tex <==
\section{ENHANCING SCALABILITY FOR SDPs WITH LOW-RANK STRUCTURE}
\label{sec:low.rank}

In this section, we focus on more scalable methods that have been developed to produce low-rank feasible solutions to the SDP in (\ref{eq:SDP}). Methods of this type are used in two different settings, which we describe now.\\

\noindent \textbf{Case 1: There is a low-rank solution among the optimal solutions to (\ref{eq:SDP}).} In this setting, we can establish a priori that among the optimal solutions to (\ref{eq:SDP}), there must be one of low rank. An important case where this is known to hold is when (\ref{eq:SDP}) does not have many constraints~\cite{pataki1998rank,lemon2016low,barvinok1995problems}. More specifically, if (\ref{eq:SDP}) has $m$ constraints and an optimal solution, then there exists a solution $X$ with rank $r$ such that 
\begin{align} \label{eq:low.rank.exist}
\frac{r(r+1)}{2} \leq m.
\end{align} Note that we need $m\leq \frac{n(n+1)}{2}$ for this property to be useful.
	
In this setting, one may not particularly care about obtaining a low-rank solution to the problem. Rather, the goal is to obtain a solution to the problem and searching for a low-rank solution (which is known to exist) can lead to significant gains in computation and storage time. To see this, recall that a $n \times n$ positive semidefinite matrix $X$ has rank $r<n$ if and only if it be written as $X=UU^T$, where $U \in \mathbb{R}^{n \times r}$. By searching for a low-rank solution, one can hope to work in the lower-dimensional space $\mathbb{R}^{n \times r}$, corresponding to $U$, rather than the higher dimensional space $\mathbb{R}^{n \times n}$, corresponding to $X$. Doing so would lead to much cheaper and faster algorithms as storage space needs would drop from $n^2$ to $nr$ numbers and matrix-vector multiplication would require $O(nr)$ flops rather than $O(n^2)$. Note though that as mentioned above, the goal in this case is to obtain \emph{optimal}---rather than simply feasible---solutions to (\ref{eq:SDP}). As a consequence, the methods we present here should hopefully produce optimal solutions when conditions such as (\ref{eq:low.rank.exist}) hold.\\

\noindent \textbf{Case 2: Good-quality low-rank feasible solutions to (\ref{eq:SDP}) are needed.} In this setting, we consider SDPs such as (\ref{eq:SDP}), whose optimal solutions may all have high rank, unlike the SDPs described in Case~1. Our goal here though is not to solve the SDP to optimality, but rather obtain low-rank feasible solutions to (\ref{eq:SDP}) with a minimum trade-off on the objective value. As we restrict ourselves to a subspace of feasible solutions with low-rank, one can also expect to work in a lower-dimensional space than the original space and make gains in terms of computation power and storage as explained previously.

Problems such as these occur in a variety of applications, most notably machine learning and combinatorial optimization. Consider for example, the max-cut problem in combinatorial optimization~ \cite{goemans1995improved}. Let $G=(V,E)$ be a simple undirected graph over $|V|=n$ nodes and recall that a \emph{cut} in the graph is a separation of the graph into two sets of nodes $S$ and $V\backslash S$, its size being given by the number of edges that link a node in $S$ to a node in $V\backslash S$. The maxcut problem involves finding the maximum cut in a given graph $G$. It can be cast as the following optimization problem 
\begin{equation}\label{eq:MAX-CUT}
\begin{aligned}
&\min_{x \in {\pm 1}^n} &&\mbox{Tr}(x^TAx),
\end{aligned}
\end{equation}
where $A$ is the adjacency matrix of the graph, which can be equivalently rewritten as the following rank-constrained SDP:
\begin{equation}\label{eq:MAX-CUT.SDP}
\begin{aligned}
&\min_{X \in S^n} &&\mbox{Tr}(AX),\\
&\text{s.t. } &&X_{ii}=1, i=1,\ldots,n\\
& && X \succeq 0, \mbox{rank}(X)=1.
\end{aligned}
\end{equation}
Such a problem though is NP-hard to solve. It is consequently relaxed to an SDP by dropping the rank constraint. Not all solutions to this SDP are valuable however: preference would be given, e.g., to a suboptimal solution of rank 1, rather than a high-rank optimal solution. This is an example of a case where methods which produce high-quality low-rank solutions would be useful. Other examples which also involve relaxing a rank-constrained SDP by dropping the rank-constraint include numerous other problems in combinatorial optimization (e.g., stable set \cite{lovasz1979shannon}, min-bisection \cite{burer2003nonlinear}) and machine learning problems (sparse PCA \cite{d2005direct}). 

One can also relax a rank-constrained SDP to an SDP by using what is known as the \emph{nuclear norm} \cite{BenMaryamPabloRank}. Consider for example the problem of low-rank matrix completion~\cite{candes2010matrix}, which is a cornerstone problem in user recommendation systems (see, e.g., the Netflix competition \cite{bennett2007netflix}). In this problem, we have access to a matrix $Z \in \mathbb{R}^{m \times n}$, which is partially complete, i.e., some of its entries are specified but others are unknown. The goal is to fill in the unknown entries. Without assuming some structure on $Z$, any completion of $Z$ would be a valid guess and so the problem is ill-defined. This can be remedied by assuming that $Z$ should have low rank, which is a natural assumption in the context of user recommender systems. Indeed, if one assumes that the matrix $Z$ reflects the ratings a user $i$ ($i=1,\ldots,n$) gives a product $j$ ($j=1,\ldots,m$), then completing the matrix $Z$ would involve infering how a user would have rated a product (s)he has not yet rated from existing ratings, provided by both him/herself and other users. Under the assumption that a consumer base can be segmented into $r$ categories (with $r\ll n$), it would then make sense to constrain the matrix $Z$ to have rank less than or equal $r$, which would reflect this segmentation. The matrix completion problem would then be written as
\begin{equation}\label{eq:matrix.completion}
\begin{aligned}
&\min_{X \in \mathbb{R}^{m \times n}} &&\sum_{i,j} (X_{ij}-Z_{ij})^2\\
&\text{s.t. } &&\mbox{rank}(X) \leq r,
\end{aligned}
\end{equation}
where $Z$ is the partially complete matrix corresponding to past data. This problem can be relaxed to an SDP by replacing the constraint on the rank of $X$ by a constraint on its nuclear norm, which is a semidefinite-representable surrogate of the rank. The problem then becomes:
\begin{equation}\label{eq:matrix.completion.relaxation}
\begin{aligned}
&\min_{X \in \mathbb{R}^{m \times n}, W_1 \in \mathbb{R}^{m \times m}, W_2 \in \mathbb{R}^{n \times n}} \sum_{i,j} (X_{ij}-Z_{ij})^2\\
&\text{s.t. } \mbox{Tr}\begin{bmatrix} W_1 & X\\ X^T & W_2 \end{bmatrix} \leq r, \begin{bmatrix} W_1 & X\\ X^T & W_2 \end{bmatrix}  \succeq 0.
\end{aligned}
\end{equation}
The goal here would be to obtain a feasible solution to the problem such that the matrix 
$$\begin{bmatrix} W_1 & X\\ X^T & W_2 \end{bmatrix}$$
has small rank. This makes matrix completion a typical application of the algorithms we present next. Other problems which involve relaxing a rank-constrained SDP to an SDP via the use of the nuclear norm include certain formulations of clustering and maximum variance unfolding \cite{kulis2007fast}.\\

The rest of this section is devoted to two of the most well-known approaches for computing low-rank feasible (and possibly optimal) solutions to the SDP in (\ref{eq:SDP}). The first one is the Burer-Monteiro method and its variants (Section \ref{subsec:BM}). The second one contains the methods that use the Frank-Wolfe algorithm as their computational backbone (Section \ref{subsec:FW}). Other methods such as the ones presented in \cite{park2016provable,bhojanapalli2016dropping} are not covered.

%
%
%Another example where the need for good-quality low-rank feasible solutions to (\ref{eq:SDP}) occurs is matrix completion and 
%
%hile optimal solutions to (\ref{eq:SDP}) may all have high rank, the only solutions that 
%
%
%	
%Such methods are usually appealing in two settings: (i) in certain situations, one can a priori establish that among the optimal solutions to (1), there must be one of low rank, (ii) in some problems, while optimal solutions to (1) may all have high rank, it may be desirable (because of the problem context) to instead search for low-rank feasible solutions with small objective value.
%
%More specifically,
%[....Explain the Barvinok bound for item (i) above.....]
%[....Give the explanation of low-rank matrix completion, and other ML and combinatorial optimization problems, where setting (ii) above arises.....]
%(So maybe you don't need a separate subsection for applications if you do it this way.)
%
%Then you move in the next paragraph to:
%
%The computational advantage of searching for low-rank solutions is that if the rank is k, then X=U*U' with U nxk. Talk about memory and computation advantages.
%
%The rest of this section is devoted to two of the most well-known approaches low-rank feasible (and possibly optimal) solutions to the SDP in (1). The first B-M. The second F-W.
%
%
%We start this section with a presentation of three examples. We will use these examples to explain how the methods presented in this section can be applied.
%
%\noindent\textbf{Example 1: An SDP with few constraints.} Consider an SDP such as (\ref{eq:SDP}):
%\begin{equation}\label{eq:SDP.bis}
%\begin{aligned}
%&\min_{X \in S_n} &&\mbox{Tr}(CX)\\
%&\text{s.t. } &&\mbox{Tr}(A_iX)=b_i,~i=1,\ldots,m\\
%& &&X \succeq 0,
%\end{aligned}
%\end{equation}
%with $m \leq \frac{n(n+1)}{2}$.
%
%\noindent \textbf{Example 2: MAX-CUT.} Let $G=(V,E)$ be a simple undirected graph over $|V|=n$ nodes. A \emph{cut} in the graph is a separation of the graph into two sets of nodes $S$ and $V\backslash S$ and its size is given by the number of edges that link a node in $S$ to a node in $V\backslash S$. The goal of this problem is to find the maximum cut in a given graph $G$ and it can be cast as the following optimization problem 
%\begin{equation}\label{eq:MAX-CUT}
%\begin{aligned}
%&\min_{x \in {\pm 1}^n} &&\mbox{Tr}(x^TAx),
%\end{aligned}
%\end{equation}
%where $A$ is the adjacency matrix of the graph. It can be equivalently rewritten as the following rank-constrained SDP:
%\begin{equation}\label{eq:MAX-CUT.SDP}
%\begin{aligned}
%&\min_{X \in S^n} &&\mbox{Tr}(AX),\\
%&\text{s.t. } &&X_{ii}=1, i=1,\ldots,n\\
%& && X \succeq 0, \mbox{rank}(X)=1.
%\end{aligned}
%\end{equation}
%
%
%
%
%
%In this section, our goal is to solve SDPs such as (\ref{eq:SDP}), but with the additional requirement that the solutions obtained should have \emph{low rank.} We call such SDPs \emph{SDPs with low-rank structure}. We recall that a $n \times n$ positive semidefinite matrix $X$ is said to have low rank if it can be written as $X=UU^T$, where $U \in \mathbb{R}^{n \times k}$, with $k \leq n$. Computationally speaking, this is a setting where one could expect fast and efficient algorithms. Indeed, one can hope to work in the lower-dimensional space $\mathbb{R}^{n \times k}$, corresponding to $U$, rather than the higher dimensional space $\mathbb{R}^{n \times n}$, corresponding to $X$. If this is done successfully, this could lead to significant gains in both storage space ($O(nk)$ bits instead of $O(n^2)$) and computation time (matrix-vector multiplication only costs $O(nk)$ bits rather than $O(n^2)$). As a consequence, this is a particularly relevant set of problems to study in the context of making SDPs more scalable. 
%
%The organization of this section is as follows: we start by reviewing areas where SDPs with low-rank structure arise in Section \ref{subsec:apps.low.rank}, and then present two popular methods for solving such problems, namely the Burer-Monteiro factorization and its variants (Section \ref{subsec:BM}) and methods based on Frank-Wolfe (Section \ref{subsec:FW}).
%
%\subsection{Applications of SDPs with low-rank structure} \label{subsec:apps.low.rank}
%
%
%
%
%
%As mentioned above, this section concerns itself with deriving solutions to SDP (\ref{eq:SDP}) that have low rank. But how can one know a priori whether an SDP has a solution that has low rank? This can in fact be deduced from the number $m$ of constraints that the SDP has. Indeed, if (\ref{eq:SDP}) has $m$ constraints and an optimal solution, then there exists a solution $X$ with rank $r$ such that $\frac{r(r+1)}{2} \leq m$ \cite{pataki1998rank,lemon2016low,barvinok1995problems}. Hence, one can apply the algorithms we present next to any SDP which has a limited number of constraints.
%
%One could argue however that SDPs 
%
%What is matrix completion: it's a problem where you have a rank constraint, which you relax into an SDP
%
%What is binary QCQP? It's a problem where you have a rank constraint together with an SDP and then you just drop the rank constraint. 
%
%In both cases, 
%
%Finally, an important class of SDPs which can be reformulated as rank-constrained SDPs are those that have very few constraints. More specifically, if the semidefinite program (\ref{eq:SDP}) has $m$ constraints and an optimal solution, then there exists a solution $X$ with rank $r$ such that $\frac{r(r+1)}{2} \leq m$~\cite{pataki1998rank,lemon2016low,barvinok1995problems}. It follows that if $r$ is the largest integer such that $\frac{r(r+1)}{2} \leq m$, then the optimization problems (\ref{eq:SDP}) and (\ref{eq:rank.SDP}) with $k=r$ are equivalent, and so one can consider (\ref{eq:rank.SDP}) instead of (\ref{eq:SDP}). 
%
%
%
%
%
%
%
% Depending on how low the rank of the solution is required to be and the structure of the SDP, one of two things can occur:
%
%
%As we discuss in more depth in Section \ref{subsec:apps.low.rank}, SDPs of this type can arise from two different venues: either the SDP is known to have a low-rank solution from the start; 
%
%In this section, we focus on optimization problems of the following form:
%\begin{equation}\label{eq:rank.SDP}
%\begin{aligned}
%&\min_{X \in S_n} &&\mbox{Tr} (CX)\\
%&\text{s.t. } &&\mbox{Tr}(A_iX)=b_i, i=1,\ldots,m\\
%& &&X \succeq 0 \text{ and } \mbox{rank}(X)\leq k,
%\end{aligned}
%\end{equation}
%where $k$, $C,A_i,b_i, i=1,\ldots,m$ are assumed known. We call problems of this type \emph{rank-constrained SDPs}. Rank-constrained SDPs are nonconvex and NP-hard to solve unlike their counterparts (\ref{eq:SDP}) obtained by dropping the rank constraint. A common approach for solving problems of this type has consequently been to relax (\ref{eq:rank.SDP}) by either dropping the rank constraint entirely or replacing it by a constraint on the nuclear norm of the matrix, which is semidefinite representable~\cite{recht2010guaranteed}. The SDP can then be solved globally using e.g. interior point methods. If the solution obtained is of appropriate rank, then it is optimal to (\ref{eq:rank.SDP}). In the case where the solution is not of appropriate rank, one can potentially use rounding methods or projection to make it feasible (though it may no longer be optimal post-processing).
%
%The line of work we present in this section is parallel to what we have described above. The algorithms we discuss here do not attempt to relax (\ref{eq:rank.SDP}) to a convex problem: they deal instead with the nonconvex optimization problem and rely on local optimization methods to do so. This of course comes with some downsides, one of them being that it can be difficult to know whether the solution obtained is a global or a local minimum. There are however some significant positives that come from leveraging the low-rank structure of the matrix from the onset as these algorithms do. Indeed, as any solution $X^*$ to (\ref{eq:rank.SDP}) can be written as $X^*=U^*U^{*T}$, where $U^* \in \mathbb{R}^{n \times k}$, we can hope to work in the lower-dimensional space $\mathbb{R}^{n \times k}$, corresponding to $U$, rather than the higher dimensional space $\mathbb{R}^{n \times n}$, corresponding to $X$. If done successfully, this could lead to significant gains in both storage space ($O(nk)$ bits instead of $O(n^2)$) and computation time (matrix-vector multiplication only costs $O(nk)$ bits rather than $O(n^2)$). 
%
%We start this section by presenting a few areas of application of rank-constrained SDPs (Section \ref{subsec:apps.low.rank}). The rest of the section will be devoted to two of the most common types of algorithms for solving rank-constrained SDPs: the Burer-Monteiro factorization and its variants (Section \ref{subsec:BM}) and methods based on the Frank-Wolfe algorithm (Section \ref{subsec:FW}).
%
%\subsection{Applications of rank-constrained SDPs} \label{subsec:apps.low.rank}
%
%Rank-constrained SDPs naturally arise in a variety of applications, particularly in machine learning. Indeed, it is often assumed---for optimization problems that arise in machine learning applications---that a solution would be low-rank, either because the problem is ill-defined without such an assumption or because it reflects some property of the model. Consider e.g. the problem of matrix completion \cite{candes2010matrix}, which is a cornerstone problem in user recommendation systems (see, e.g., the Netflix prize). In this problem, we have access to a matrix $Z \in \mathbb{R}^{m \times n}$, which is partially complete, i.e., some of its entries are specified but others are unknown. The goal is to fill in the unknown entries. Without assuming some structure on $Z$, any completion of $Z$ would be a valid guess and so the problem is ill-defined. This can be remedied by assuming that $Z$ should have low rank. In the context of user recommender systems, this assumption is actually quite natural. Indeed, if one assumes that the matrix $Z$ reflects the ratings a user $i$ ($i=1,\ldots,n$) gives a product $j$ ($j=1,\ldots,m$), then completing the matrix $Z$ would involve infering how a user would have rated a product from existing ratings. Under the assumption that a consumer base can be segmented into $k$ categories, it would then make sense to constrain the matrix $Z$ to have rank less than or equal $k$, which would reflect this segmentation. The matrix completion problem would then be written
%\begin{equation}\label{eq:matrix.completion}
%\begin{aligned}
%&\min_{X \in \mathbb{R}^{m \times n}} &&\sum_{i,j} (X_{ij}-Z_{ij})^2\\
%&\text{s.t. } &&\mbox{rank}(X) \leq k,
%\end{aligned}
%\end{equation}
%where $Z$ is the partially complete matrix corresponding to past data. Similarly, clustering and maximum variance unfolding can be cast as rank-constrained SDPs \cite{kulis2007fast}.
%
%Rank-constrained SDPs also appear as reformulations of quadratically constrained quadratic programs with binary constraints. Consider for example the following quadratically constrained quadratic program with binary constraints:
%\begin{equation}\label{eq:QCQP.bin}
%\begin{aligned}
%&\min_{x \in \{-1,1\}^n} &&x^TCx\\
%&\text{s.t. } &&x^TA_i x \leq b_i, i=1,\ldots,m.
%\end{aligned}
%\end{equation}
%This problem can be rewritten as 
%\begin{equation} \label{eq:SDP.rank1}
%\begin{aligned}
%&\min_{X \in S^{n \times n}} &&\mbox{Tr}(CX)\\
%&\text{s.t. } &&\mbox{Tr}(A_iX) \leq b_i, i=1,\ldots,m\\
%& &&X \succeq 0, X_{ii}=1, i=1,\ldots,m \text{ and } \mbox{rank}(X)=1,
%\end{aligned}
%\end{equation}
%which is a rank-constrained SDP. Problems that can be cast in such a way include combinatorial optimization problems (stable set \cite{lovasz1979shannon}, max-cut \cite{goemans1995improved}, min-bisection \cite{burer2003nonlinear}) and machine learning problems (sparse PCA \cite{d2005direct}).
%
%Finally, an important class of SDPs which can be reformulated as rank-constrained SDPs are those that have very few constraints. More specifically, if the semidefinite program (\ref{eq:SDP}) has $m$ constraints and an optimal solution, then there exists a solution $X$ with rank $r$ such that $\frac{r(r+1)}{2} \leq m$~\cite{pataki1998rank,lemon2016low,barvinok1995problems}. It follows that if $r$ is the largest integer such that $\frac{r(r+1)}{2} \leq m$, then the optimization problems (\ref{eq:SDP}) and (\ref{eq:rank.SDP}) with $k=r$ are equivalent, and so one can consider (\ref{eq:rank.SDP}) instead of (\ref{eq:SDP}). 
%
%
%
%%Most frequently however, SDPs with low-rank solutions are in fact relaxations of optimization problems with low-rank constraints. Consider for example the following quadratically constrained quadratic program with binary constraints:
%%\begin{equation}\label{eq:QCQP.bin}
%%\begin{aligned}
%%&\min_{x \in \{-1,1\}^n} &&x^TCx\\
%%&\text{s.t. } &&x^TA_i x \leq b_i, i=1,\ldots,m.
%%\end{aligned}
%%\end{equation}
%%This problem can be rewritten as 
%%\begin{equation} \label{eq:SDP.rank1}
%%\begin{aligned}
%%&\min_{X \in S^{n \times n}} &&\mbox{Tr}(CX)\\
%%&\text{s.t. } &&\mbox{Tr}(A_iX) \leq b_i, i=1,\ldots,m\\
%%& &&X \succeq 0, X_{ii}=1, i=1,\ldots,m \text{ and } \mbox{rank}(X)=1,
%%\end{aligned}
%%\end{equation}
%%which is a rank-constrained optimization problem. Problems of this type appear in many different applications, particularly in combinatorial optimization (stable set \cite{lovasz1979shannon}, max-cut \cite{goemans1995improved}, min-bisection \cite{burer2003nonlinear}) and machine learning (sparse PCA \cite{d2005direct}). Note that in this case, the rank constraint appears as an artefact of the rewriting of (\ref{eq:QCQP.bin}). It can also be the case that the presence of a rank constraint is endogenous to the problem. This is often the case in machine learning, for example, where it is necessary to assume that a solution is low rank, either because the problem is ill-defined without such an assumption or because it reflects some property of the model. Consider e.g. the problem of matrix completion \cite{candes2010matrix}, which is a cornerstone problem in user recommendation systems (see, e.g., the Netflix prize). In this problem, we have access to a matrix $Z \in \mathbb{R}^{m \times n}$, which is partially complete, i.e., some of its entries are specified but others are unknown. The goal is to fill in the unknown entries. Without assuming some structure on $Z$, any completion of $Z$ would be a valid guess and so the problem is ill-defined. This can be remedied by assuming that $Z$ should have low rank. In the context of user recommender systems, this assumption is actually quite natural. Indeed, if one assumes that the matrix $Z$ reflects the ratings a user $i$ ($i=1,\ldots,n$) gives a product $j$ ($j=1,\ldots,m$), then completing the matrix $Z$ would involve infering how a user would have rated a product from existing ratings. Under the assumption that a consumer base can be segmented into $k$ categories (which is a common assumption in marketing), it would then make sense to constrain the matrix $Z$ to have rank less than or equal $k$, which would reflect this segmentation. The matrix completion problem would then be written
%%\begin{equation}\label{eq:matrix.completion}
%%\begin{aligned}
%%&\min_{X \in \mathbb{R}^{m \times n}} &&\sum_{i,j} (X_{ij}-Z_{ij})^2\\
%%&\text{s.t. } &&\mbox{rank}(X) \leq k,
%%\end{aligned}
%%\end{equation}
%%where $Z$ is the partially complete matrix corresponding to past data. Similar examples that arise in machine learning include clustering and maximum variance unfolding \cite{kulis2007fast}.
%
%%
%%
%%[*Something about the algorithms we are going to present are tailored to exactly problems of the form (2). They are NP-hard to solve so some research interest has gone into providing good relaxations for them (nuclear norm etc). This is not what we're doing here. Here, $k$ is very much a parameter of the problem. It is worth mentioning that ]
%%
%%
%%Note that neither (\ref{eq:SDP.rank1}) nor (\ref{eq:matrix.completion}) are SDPs; in fact, they are NP-hard to solve. To obtain SDPs, one needs to relax the initial problems by either dropping the rank constraint (typically, for problems such as (\ref{eq:SDP.rank1})), or by replacing the rank constraint on the matrix by a constraint on its nuclear norm \cite{recht2010guaranteed}. For example, in the case of (\ref{eq:matrix.completion}), the problem could be relaxed to
%%\begin{equation}\label{eq:matrix.completion.relaxation}
%%\begin{aligned}
%%&\min_{X \in \mathbb{R}^{m \times n}, W_1 \in \mathbb{R}^{m \times m}, W_2 \in \mathbb{R}^{n \times n}} \sum_{i,j} (X_{ij}-Z_{ij})^2\\
%%&\text{s.t. } \mbox{Tr}\begin{bmatrix} W_1 & X\\ X^T & W_2 \end{bmatrix} \leq k, \begin{bmatrix} W_1 & X\\ X^T & W_2 \end{bmatrix}  \succeq 0.
%%\end{aligned}
%%\end{equation}
%%[*Say something about the two methods here* Burer Monteiro doesn't require dropping the rank constraint as it is hard-coded into the problem as we see next.*]

\subsection{Burer-Monteiro-based methods} \label{subsec:BM}
The key idea of the Burer-Monteiro algorithm \cite{burer2003nonlinear} is to factor the decision variable $X$ in (\ref{eq:SDP}) as $VV^T$ where $V \in \mathbb{R}^{n \times r}$. Here, $r$ can either be chosen such that a solution of rank $r$ is guaranteed to exist (e.g., such that (\ref{eq:low.rank.exist}) holds) (Case 1) or such that it corresponds to the rank which we would like our solution to be (Case 2). Typically, the algorithm comes with theoretical guarantees for the first case and is simply a heuristic in the second case. Using this factorization, we rewrite (\ref{eq:SDP}) as:
\begin{equation}\label{eq:BM}
\begin{aligned}
&\min_{V \in \mathbb{R}^{n \times r}} &&\mbox{Tr}(CVV^T)\\
&\text{s.t. } &&\mbox{Tr}(A_iVV^T)=b_i, i=1,\ldots,m.
\end{aligned}
\end{equation}
This reformulation has both pros and cons: on the upside, the problem to consider has smaller dimension than (\ref{eq:SDP}) and has no conic constraint to contend with; on the downside, the problem becomes nonconvex. Hence, local optimization methods may not always recover the global minimum of (\ref{eq:SDP}) even if a low-rank solution is known to exist. Research in this area has consequently sought to find an algorithm to solve (\ref{eq:BM}) that (i) provably recovers global low-rank solutions to the problem if they exist; (ii) does so reasonably fast both in terms of convergence rates and experimentally; and (iii) works on a large class of inputs $A_i, b_i,$ and $C$. We review existing algorithms through the lense of these criteria.

\subsubsection{Augmented Lagrangian approaches}
The method recommended by Burer and Monteiro themselves to solve (\ref{eq:BM}) is a method based on an augmented Lagrangian procedure \cite{burer2003nonlinear} (see Section \ref{subsec:Aug.Lag.Method} for another appearance of this general approach). The idea is to rewrite (\ref{eq:BM}) as an unconstrained optimization problem by adding terms to the objective that penalize infeasible points. This is done by constructing an augmented Lagrangian function, given here by
$$L_{y,\sigma}(V)=\mbox{Tr}(CVV^T)-\sum_{i=1}^m y_i (\mbox{Tr}(A_iVV^T)-b_i)+\frac{\sigma}{2} \sum_{i=1}^m (\mbox{Tr}(A_iVV^T)-b_i)^2.$$
If $y$ and $\sigma >0$ are fixed appropriately, then minimizing $L_{y,\sigma}(\cdot)$ will yield an optimal solution to (\ref{eq:BM}). To obtain an appropriate pair $(y,\sigma)$, the following iterative procedure is followed: fix $(y,\sigma)$ and minimize $L_{y,\sigma}(\cdot)$ to obtain $V$, then construct a new $(y,\sigma)$ from $V$, and repeat; see \cite{burer2003nonlinear} for the exact details. Note that this procedure involves the minimization of $L_{y,\sigma}$ with respect to $V$: choosing an appropriate algorithm for this subproblem is also an important step in the method. The authors in \cite{burer2003nonlinear} suggest using a limited-memory BFGS (LM-BFGS) algorithm \cite{liu1989limited} to do so. The LM-BFGS algorithm is a quasi-Newton algorithm for unconstrained optimization problems, where the objective is differentiable. Unlike Newton methods, it does not require computing the Hessian of the objective function, constructing instead an approximate representation of it from past gradients. Given that gradients of $L_{y,\sigma}$ can be computed quite quickly under some conditions (see \cite{burer2003nonlinear} for more details), this is a reasonably efficient algorithm to use. One can replace the LM-BFGS subroutine with a subgradient approach if (\ref{eq:BM}) has additional constraints that are non-differentiable. Furthermore, the augmented Lagrangian approach has been tailored to directly handle inequality constraints of the type $\mbox{Tr}(A_iX) \leq b_i$ in (\ref{eq:SDP}). Though there are no theoretical guarantees regarding convergence to global solutions, the authors of \cite{burer2003nonlinear} experimentally observe that the algorithm tends to return global minima, doing so in a much smaller amount of time than interior point or bundle methods. The follow-up paper \cite{burer2005local} to \cite{burer2003nonlinear} slightly modifies the augmented Lagrangian function and shows convergence of the algorithm to a global minimum (given that one exists of rank $\leq r$) if, among other things, each minimization of the modified $L_{y,\sigma}(\cdot)$ gives rise to a local minimum, something that is hard to test in practice.

\subsubsection{Riemannian optimization algorithms}
Riemannian optimization concerns itself with the optimization of a smooth objective function over a smooth Riemannian manifold. We remind the reader that a \emph{Riemannian} manifold $\mathcal{M}$ is a manifold that can be linearized at each point $x \in \mathcal{M}$ by a tangent space $T_x \mathcal{M}$, which is equipped with a Riemannian metric. We say that a Riemannian manifold is \emph{smooth} if the Riemannian metric varies smoothly as the point $x$ varies; see e.g. \cite[Appendix A]{boumal2011rtrmc} for a short introduction to such concepts.  In the Riemannian setting, one can define notions of both gradients and Hessians for manifolds \cite[Appendix A]{boumal2011rtrmc}. Using these notions, one can extend the concepts of first-order and second-order necessary conditions of optimality to optimization over manifolds. These are identical to the ones for unconstrained optimization over $\mathbb{R}^n$, except that they involve the analogs of gradient and Hessians for manifolds. Similarly, one can generalize many classical algorithms for nonlinear unconstrained optimization (such as, e.g., trust-region and gradient-descent methods) to the manifold setting. We refer the reader to \cite{absil2007trust,absil2009optimization} for more information on the specifics of these algorithms which we will not cover here.

Though it may not be immediately apparent as to why, Riemannian optimization methods have become a popular tool for tackling problems of the form (\ref{eq:BM}) \cite{journee2010low,boumal2016non}. Indeed, the set
$$\mathcal{M}=\{V \in \mathbb{R}^{n \times r}~|~\mbox{Tr}(A_iVV^T)=b_i, i=1,\ldots,m\}$$
is a smooth Riemannian manifold under certain conditions on $A_i$ (see \cite[Assumption 1]{boumal2018deterministic}), and the objective function $V \mapsto \mbox{Tr}(CVV^T)$ is smooth. Hence, (\ref{eq:BM}) is exactly a Riemannian optimization problem. It can be shown that if $m < \frac{r(r+1)}{2}$, the conditions on $\mathcal{M}$ that make it smooth hold, and $\mathcal{M}$ is compact, then for almost all $C \in S_n$, any second-order critical point of (\ref{eq:BM}) is globally optimal to (\ref{eq:SDP}) \cite[Theorem 2]{boumal2016non}. (Note that an optimal solution of rank $\leq k$ is guaranteed to exist here from the assumptions and that we use the manifold definition of a second-order critical point.) If an algorithm which returns second-order critical points can be exhibited, then, in effect, we will have found a way of solving (\ref{eq:BM}). It so happens that the Riemannian trust-region method returns such a point---under some conditions---regardless of initialization \cite{boumal2018global}. In fact, it is shown in \cite{boumal2018global} that an $\epsilon$-accurate second-order critical point (i.e., a point $V \in \mathcal{M}$ with $||\mbox{grad}(\mbox{Tr}(CVV^T))|| \leq \epsilon$ and $\mbox{Hessian}(\mbox{Tr}(CVV^T)) \succeq -\epsilon I$ ) can be obtained in $O(1/\epsilon^2)$ iterations. This makes the Riemannian trust-region problem a popular algorithm to use among all possible algorithms one could use to solve (\ref{eq:BM}) (Riemannian or otherwise) as it has good theoretical guarantees. Other Riemannian methods which come with some theoretical guarantees are the Riemannian steepest-descent algorithm and the Riemannian conjugate gradient algorithm, both of them being known to converge to a critical point of (\ref{eq:BM}) \cite{boumal2018global, sato2015new}. In practice however, many more algorithms for nonlinear optimization can be and have been generalized to manifold settings (though their convergence properties have not necessarily been studied) and are used to solve problems such as (\ref{eq:BM}) (see, e.g., the list of solvers implemented in MANOPT, one of the main toolboxes for optimization over manifolds \cite{manopt}). 

We conclude this section by mentioning a few applications where Riemannian optimization methods have recently been used. These include machine learning problems such as synchronization \cite{mei2017solving}, phase recovery \cite{sun2018geometric}, dictionary learning \cite{sun2016complete}, and low-rank matrix completion \cite{boumal2011rtrmc}; but also robotics problems such as the \emph{Simultaneous Localization and Mapping (SLAM)} problem. SLAM \cite{probabilistic robotics} refers to the problem of simultaneously estimating the location (or trajectory of locations) of a robot and a model of the robot's environment. Two important versions of the SLAM problem are (i) Landmark SLAM, and (ii) Pose-graph SLAM. The Landmark SLAM problem involves simultaneously estimating the position and orientation of the robot and the location of landmarks in the environment. The Pose-graph SLAM problem is a more restricted version that only requires estimating the position and orientation of the robot at each time-step. Traditionally, these problems have been posed as maximum likelihood estimation (MLE) problems and tackled using general nonlinear optimization methods (which do not come with guarantees on finding globally optimal solutions). % \cite{8-14-15-16-ram}. 
More recently, researchers have proposed semidefinite programming relaxations for the MLE problem arising from SLAM \cite{sesync, 25-27-sesync, 4-6-7-ram}. These relaxations provide exact solutions to the MLE problem assuming that noise in the measurements made by the robot are below a certain threshold (see \cite{se-sync} for exact conditions). In \cite{se-sync}, the authors demonstrate that the resulting SDP admits low-rank solutions and use a Burer Monteiro factorization combined with Riemannian optimization techniques (e.g., a Riemannian trust-region approach)  to solve the SDP. Thus, assuming that the conditions on the measurement noise are satisfied, one can find globally optimal solutions to the MLE problems arising from Pose-graph SLAM (and other related MLE problems arising from camera motion estimation and sensor network localization problems) via this method.

\subsubsection{Coordinate descent approaches}

One of the more recent trends for solving problems of the form (\ref{eq:BM}) has been to use coordinate descent (or block-coordinate descent) methods \cite{erdogdu2018convergence,wang2017mixing}. They come with the caveat that they can only be used to solve diagonally-constrained problems, i.e., problems of the type
\begin{equation}\label{eq:diag.constr}
\begin{aligned}
&\min_{V \in \mathbb{R}^{n \times r}} &&\mbox{Tr}(CVV^T)\\
&\text{s.t. } &&||v_i^T||_2=b_i, i=1,\ldots,n.
\end{aligned}
\end{equation}
where $||\cdot||_2$ is the 2-norm and $v_i^T$ is the $i^{th}$ row of $V$. Note that, e.g., the max-cut problem fits into this framework. Coordinate-descent methods are easy to explain for this case. Let us assume that $b_i=1$ for $i=1,\ldots,m$ for clarity of exposition. Initialization consists in randomly choosing $v_i, i=1,\ldots,n$ on the sphere. Then, at each iteration, an index $i$ is picked and fixed, and the goal is to find a vector $v_i$ such that $\mbox{Tr}(CVV^T)=\sum_{i,j=1}^n c_{ij}v_iv_j^T$ is minimum. As $||v_i||=1$, it follows that we can replace $c_{ii}$ by $0$ without changing the optimal solution. The problem then is equivalent to minimizing $v_i^T(\sum_{j=1}^n c_{ij}v_j)$ for $||v_i||=1$ and admits a closed form solution:
$$v_i=-\frac{\sum_{j=1}^n c_{ij}v_j}{||\sum_{j=1}^n c_{ij}v_j||}.$$
We update the objective by replacing the previous $v_i$ by this new $v_i$ and proceed to the next iteration. This algorithm can be slightly modified to consider descent on blocks of coordinates, rather than one single coordinate at each time-step \cite{erdogdu2018convergence}. In that setting, it can be shown that if the indexes are picked in a correct way, then coordinate block-descent methods converge to an $\epsilon$-accurate critical point of (\ref{eq:BM}) in time $O(\frac{1}{\epsilon})$. Each iteration of coordinate descent methods is much less costly (by an order of $n$ approximately)  than its Riemannian trust region counterpart however. As a consequence, numerical results tend to show that as $n$ increases, using coordinate descent methods can be preferable \cite{erdogdu2018convergence}.

\subsection{Frank-Wolfe based methods} \label{subsec:FW}

We start this subsection by a quick presentation of the Frank-Wolfe algorithm (also known as the conditional gradient algorithm), a version of which will be used in the algorithms we present. The Frank-Wolfe algorithm was first proposed in a seminal paper by Frank and Wolfe in 1956 \cite{frank1956algorithm}. It is an algorithm for constrained optimization problems of the type $\min_{x \in S} f(x)$, where $S$ is compact and convex and $f$ is convex and differentiable. At each step $k$, a linear approximation of $f$ (obtained by taking the first-order Taylor approximation of $f$ around the current iterate $x_k$) is minimized over $S$ and a minimizer $s_k$ is obtained. The next iterate $x_{k+1}$ is then constructed by taking a convex combination of the previous iterate $x_k$ and the minimizer $s_k$ before repeating the process. Intuitively, the reason why Frank Wolfe algorithms are popular for obtaining low-rank feasible solutions for SDPs is due to the following fact: if the algorithm is initialized with a rank-1 matrix and if each minimizer is also a rank-1 matrix, then the $k^{th}$ iterate is of rank at most $k$. This enables us to control the rank of the solution that is given as output. We first present an algorithm developed by Hazan \cite{hazan2008sparse} in Section \ref{subsec:Hazan} and follow up with some extensions of Hazan's algorithm in Section \ref{subsec:other.FW}.

\subsubsection{Hazan's algorithm} \label{subsec:Hazan}
Hazan's algorithm is an algorithm which is designed to produce low-rank solutions to SDPs of the type
\begin{equation}\label{eq:SDP.compact}
\begin{aligned}
&\min_{X \in S_n} &&\mbox{Tr}(CX)\\
&\text{s.t. } &&\mbox{Tr}(A_iX)=b_i,~i=1,\ldots,m\\
& &&X \succeq 0 \text{ and } \mbox{Tr}(X)=1.
\end{aligned}
\end{equation}
Note the presence of the additional constraint $\mbox{Tr}(X)=1$, which restricts the applicability of this method. The constraint on the trace can be slightly relaxed to $\mbox{Tr}(X)\leq t$, where $t$ is fixed \cite[Chapter 5]{gartner2012approximation}, but we will consider the case $\mbox{Tr}(X)=1$ here. A key subroutine of Hazan's algorithm is solving the following optimization problem:
\begin{equation}\label{eq:Hazan}
\begin{aligned}
&\min_{X \in S_n} &&f(X)\\
&\text{s.t. } &&\mbox{Tr}(X)=1 \text{ and } X\succeq 0,
\end{aligned}
\end{equation}
where $f$ is a convex function. Let $f^*$ be the optimal value of this problem. It is for this subroutine that a Frank-Wolfe type iterative algorithm is used. It can be described as follows: initalize $X_1$ to be a rank $1$ matrix with trace one. Then, at iteration $k$, compute the eigenvector $v_k$ corresponding to the maximum eigenvalue of $\nabla f(X_k)$. Finally, for a fixed parameter $\alpha_k$, set $X_{k+1}=(1-\alpha_k)X_k+\alpha_k (-v_kv_k^T)$ and reiterate. This algorithm returns a $\frac{1}{k}$-approximate solution (i.e., a matrix $X$ such that $\mbox{Tr}(X) \leq 1+\frac{1}{k}$ and $f(X) \leq f^*+\Omega(\frac{1}{k})$) with rank at most $k$ in $k$ iterations. This is of interest in itself as some problems can be cast in the form (\ref{eq:Hazan}), an example being given in \cite{hazan2008sparse}.

It can also be used, as mentioned previously, to solve (\ref{eq:SDP.compact}). To see how this is done, first note that one can reduce solving (\ref{eq:SDP.compact}) to solving a sequence of SDP feasibility problems via the use of bisection. It is enough as a consequence to explain how one can leverage the Frank-Wolfe type algorithm described above to solve an SDP feasibility problem of the type: $\mbox{Tr}(A_iX) \leq b_i,i=1,\ldots,m, X\succeq 0, \mbox{Tr}(X)=1$. Quite straightforwardly, this can be done by letting $f(X)=\frac{1}{M} \log(\sum_{i=1}^m e^{M\cdot (\mbox{Tr}(A_iX)-b_i)})$ where $M=k\log(m)$, $\frac{1}{k}$ being the desired accuracy; see \cite{hazan2008sparse}. The algorithm is then guaranteed to return a $\frac{1}{k}$-approximate solution of rank at most $k$ in $O(k^2)$ iterations.

It is interesting to note that this latter algorithm is nearly identical to the Multiplicative Weights algorithm for SDPs which also produces low-rank solutions \cite{arora2012multiplicative} and has exactly the same guarantees. However it is derived in a completely different fashion.

\subsubsection{Other methods based on Frank-Wolfe} \label{subsec:other.FW}
A caveat of Hazan's algorithm is that the rank of the solution returned is linked to its accuracy. One could maybe think that, as the solution is known to be low-rank and the Frank-Wolfe algorithm is initialized with a low-rank matrix, then all iterates of the algorithm would be low-rank, and so one could hope to have rank guarantees on the iterates, regardless of the number of iterations. Unfortunately it is not the case that all iterates have low rank. In fact, what can be observed in practice is that the Frank-Wolfe algorithm typically returns iterates with increasing rank up to a certain point, where the rank decreases again, with the final solution returned being low-rank; see, e.g., the numerical experiments in \cite{yurtsever2017sketchy}. As a consequence, if one requires an accurate solution, one will likely have to deal with high-rank intermediate iterates, with the storage and computational problems that this entails.

In this section, we present two different methods designed to avoid these issues. To the best of our knowledge, these methods only apply to a specific class of optimization problems of the type:
\begin{equation}\label{eq:app.FW}
\begin{aligned}
&\min_{X \in \mathbb{R}^{n \times d}} f(\mathcal{A}X)\\
&\text{s.t. } ||X||_{N}\leq 1,
\end{aligned}
\end{equation}
where $f$ is a convex and differentiable function, $||\cdot||_N$ is the nuclear norm of the matrix $X$ \cite{BenMaryamPabloRank}, and $\mathcal{A}:\mathbb{R}^{n\times d} \rightarrow \mathbb{R}^m$ is a linear operator, mapping $X$ to $[\mbox{Tr}(A_1X),\ldots,\mbox{Tr}(A_mX)]$. Note that e.g. the relaxation of the low-rank matrix completion problem given in (\ref{eq:matrix.completion.relaxation}) fits into this format. Similarly to (\ref{eq:Hazan}), the Frank-Wolfe algorithm can be applied to (\ref{eq:app.FW}) quite readily. Initialization is done as before by setting $X_0$ to be some rank-1 matrix. At iteration $k$, one computes an update direction by finding a pair $(u_k,v_k)$ of singular vectors corresponding to the maximum singular value of $
\mathcal{A}^*( \nabla f(\mathcal{A}X_k))$ where $\mathcal{A}^*:\mathbb{R}^m \mapsto \mathbb{R}^{n \times d}$ is the dual linear operator to $\mathcal{A}$ given by $\mathcal{A}^*z=\sum_{i=1}^m z_i A_i$. We then construct a new iterate $X_{k+1}=(1-\alpha)X_k-\alpha u_kv_k^T$ and repeat.

The first method, described in \cite{freund2017extended}, is a modification of the Frank-Wolfe algorithm as described in the previous paragraph. The key idea is that at every iteration, the algorithm chooses between two types of steps. One type is the step described above, which is derived from the singular vectors of the matrix, (a ``regular'' step in the paper); the other is what is called an ``in-face step''. These can be constructed in different ways, but one way of doing this is to minimize $\mathcal{A}^*(\nabla f(\mathcal{A}X_k))$ over the minimal face of the nuclear norm unit ball to which $X_k$ belongs. The matrix $Z_k$ obtained is then used to produce the next iterate: $X_{k+1}=(1-\alpha)X_k+\alpha Z_k$. We refer the reader to \cite{freund2017extended} to see how this can be done efficiently. The advantage of such a step is that the matrix $X_{k+1}$ constructed has rank no larger than $X_k$. If the choice between a regular step and an away step is appropriately made, it can still be the case that one has a $\frac{1}{k}$-approximate solution after $k$ iterations, though the rank of the $k^{th}$ iterate could be much less than $k$ depending on the amount of ``in face'' steps used.

The second method given in \cite{yurtsever2017sketchy} describes an alternative way of dealing with the intermediate iterates $X_k$. To get around this problem, the authors devise a ``dual'' formulation of the Frank-Wolfe algorithm described above where the primal iterates $X_k \in \mathbb{R}^{n \times d}$ are replaced by dual iterates $z_k \in \mathbb{R}^m$, which are of smaller size, thus reducing the computation time. There is a need however to keep track of the iterates $X_k$ in some sense as the ultimate goal is to recover a solution at the end of the algorithm. To do this, the authors suggest a procedure that they call \emph{sketching}. The procedure is as follows: two random matrices $\Omega \in \mathbb{R}^{n \times j}$ and $\Psi \in \mathbb{R}^{l \times d}$ are generated such that $j$ and $l$ are of order of the rank $r$ of the solution to (\ref{eq:app.FW}), and two new matrices $Y$ and $W$ are obtained by projecting $X$ onto $\Omega$ and $\Psi$, i.e., $Y=X\Omega$ and $W=\Psi X$. Note that the matrices $(Y,W)$ typically have smaller rank than the iterates $X_k$ that they represent. Any update that is made in the algorithm is then reflected on $(Y,W)$ rather than on the matrix $X$. At the end of the algorithm, one can reconstruct a rank $r$ solution to the problem from the updated pair $(Y,W)$; see \cite{yurtsever2017sketchy} for details. Note that with this way of proceeding, one need never store or use for computation full-rank intermediate iterates.

==> sections/low_rank_old.tex <==
\section{SCALABLE ALGORITHMS FOR RANK-CONSTRAINED SDPs}
\label{sec:low.rank}

In this section, we focus on optimization problems of the following form:
\begin{equation}\label{eq:rank.SDP}
\begin{aligned}
&\min_{X \in S_n} &&\mbox{Tr} (CX)\\
&\text{s.t. } &&\mbox{Tr}(A_iX)=b_i, i=1,\ldots,m\\
& &&X \succeq 0 \text{ and } \mbox{rank}(X)\leq k,
\end{aligned}
\end{equation}
where $k$, $C,A_i,b_i, i=1,\ldots,m$ are assumed known. We call problems of this type \emph{rank-constrained SDPs}. Rank-constrained SDPs are nonconvex and NP-hard to solve unlike their counterparts (\ref{eq:SDP}) obtained by dropping the rank constraint. A common approach for solving problems of this type has consequently been to relax (\ref{eq:rank.SDP}) by either dropping the rank constraint entirely or replacing it by a constraint on the nuclear norm of the matrix, which is semidefinite representable~\cite{BenMaryamPabloRank}. The SDP can then be solved globally using e.g. interior point methods. If the solution obtained is of appropriate rank, then it is optimal to (\ref{eq:rank.SDP}). In the case where the solution is not of appropriate rank, one can potentially use rounding methods or projection to make it feasible (though it may no longer be optimal post-processing).

The line of work we present in this section is parallel to what we have described above. The algorithms we discuss here do not attempt to relax (\ref{eq:rank.SDP}) to a convex problem: they deal instead with the nonconvex optimization problem and rely on local optimization methods to do so. This of course comes with some downsides, one of them being that it can be difficult to know whether the solution obtained is a global or a local minimum. There are however some significant positives that come from leveraging the low-rank structure of the matrix from the onset as these algorithms do. Indeed, as any solution $X^*$ to (\ref{eq:rank.SDP}) can be written as $X^*=U^*U^{*T}$, where $U^* \in \mathbb{R}^{n \times k}$, we can hope to work in the lower-dimensional space $\mathbb{R}^{n \times k}$, corresponding to $U$, rather than the higher dimensional space $\mathbb{R}^{n \times n}$, corresponding to $X$. If done successfully, this could lead to significant gains in both storage space ($O(nk)$ bits instead of $O(n^2)$) and computation time (matrix-vector multiplication only costs $O(nk)$ bits rather than $O(n^2)$). 

We start this section by presenting a few areas of application of rank-constrained SDPs (Section \ref{subsec:apps.low.rank}). The rest of the section will be devoted to two of the most common types of algorithms for solving rank-constrained SDPs: the Burer-Monteiro factorization and its variants (Section \ref{subsec:BM}) and methods based on the Frank-Wolfe algorithm (Section \ref{subsec:FW}).

\subsection{Applications of rank-constrained SDPs} \label{subsec:apps.low.rank}

Rank-constrained SDPs naturally arise in a variety of applications, particularly in machine learning. Indeed, it is often assumed---for optimization problems that arise in machine learning applications---that a solution would be low-rank, either because the problem is ill-defined without such an assumption or because it reflects some property of the model. Consider e.g. the problem of matrix completion \cite{candes2010matrix}, which is a cornerstone problem in user recommendation systems (see, e.g., the Netflix prize). In this problem, we have access to a matrix $Z \in \mathbb{R}^{m \times n}$, which is partially complete, i.e., some of its entries are specified but others are unknown. The goal is to fill in the unknown entries. Without assuming some structure on $Z$, any completion of $Z$ would be a valid guess and so the problem is ill-defined. This can be remedied by assuming that $Z$ should have low rank. In the context of user recommender systems, this assumption is actually quite natural. Indeed, if one assumes that the matrix $Z$ reflects the ratings a user $i$ ($i=1,\ldots,n$) gives a product $j$ ($j=1,\ldots,m$), then completing the matrix $Z$ would involve infering how a user would have rated a product from existing ratings. Under the assumption that a consumer base can be segmented into $k$ categories, it would then make sense to constrain the matrix $Z$ to have rank less than or equal $k$, which would reflect this segmentation. The matrix completion problem would then be written
\begin{equation}\label{eq:matrix.completion}
\begin{aligned}
&\min_{X \in \mathbb{R}^{m \times n}} &&\sum_{i,j} (X_{ij}-Z_{ij})^2\\
&\text{s.t. } &&\mbox{rank}(X) \leq k,
\end{aligned}
\end{equation}
where $Z$ is the partially complete matrix corresponding to past data. Similarly, clustering and maximum variance unfolding can be cast as rank-constrained SDPs \cite{kulis2007fast}.

Rank-constrained SDPs also appear as reformulations of quadratically constrained quadratic programs with binary constraints. Consider for example the following quadratically constrained quadratic program with binary constraints:
\begin{equation}\label{eq:QCQP.bin}
\begin{aligned}
&\min_{x \in \{-1,1\}^n} &&x^TCx\\
&\text{s.t. } &&x^TA_i x \leq b_i, i=1,\ldots,m.
\end{aligned}
\end{equation}
This problem can be rewritten as 
\begin{equation} \label{eq:SDP.rank1}
\begin{aligned}
&\min_{X \in S^{n \times n}} &&\mbox{Tr}(CX)\\
&\text{s.t. } &&\mbox{Tr}(A_iX) \leq b_i, i=1,\ldots,m\\
& &&X \succeq 0, X_{ii}=1, i=1,\ldots,m \text{ and } \mbox{rank}(X)=1,
\end{aligned}
\end{equation}
which is a rank-constrained SDP. Problems that can be cast in such a way include combinatorial optimization problems (stable set \cite{lovasz1979shannon}, max-cut \cite{goemans1995improved}, min-bisection \cite{burer2003nonlinear}) and machine learning problems (sparse PCA \cite{dAspremont07}).

Finally, an important class of SDPs which can be reformulated as rank-constrained SDPs are those that have very few constraints. More specifically, if the semidefinite program (\ref{eq:SDP}) has $m$ constraints and an optimal solution, then there exists a solution $X$ with rank $r$ such that $\frac{r(r+1)}{2} \leq m$~\cite{pataki1998rank,lemon2016low,barvinok1995problems}. It follows that if $r$ is the largest integer such that $\frac{r(r+1)}{2} \leq m$, then the optimization problems (\ref{eq:SDP}) and (\ref{eq:rank.SDP}) with $k=r$ are equivalent, and so one can consider (\ref{eq:rank.SDP}) instead of (\ref{eq:SDP}). 



%Most frequently however, SDPs with low-rank solutions are in fact relaxations of optimization problems with low-rank constraints. Consider for example the following quadratically constrained quadratic program with binary constraints:
%\begin{equation}\label{eq:QCQP.bin}
%\begin{aligned}
%&\min_{x \in \{-1,1\}^n} &&x^TCx\\
%&\text{s.t. } &&x^TA_i x \leq b_i, i=1,\ldots,m.
%\end{aligned}
%\end{equation}
%This problem can be rewritten as 
%\begin{equation} \label{eq:SDP.rank1}
%\begin{aligned}
%&\min_{X \in S^{n \times n}} &&\mbox{Tr}(CX)\\
%&\text{s.t. } &&\mbox{Tr}(A_iX) \leq b_i, i=1,\ldots,m\\
%& &&X \succeq 0, X_{ii}=1, i=1,\ldots,m \text{ and } \mbox{rank}(X)=1,
%\end{aligned}
%\end{equation}
%which is a rank-constrained optimization problem. Problems of this type appear in many different applications, particularly in combinatorial optimization (stable set \cite{lovasz1979shannon}, max-cut \cite{goemans1995improved}, min-bisection \cite{burer2003nonlinear}) and machine learning (sparse PCA \cite{d2005direct}). Note that in this case, the rank constraint appears as an artefact of the rewriting of (\ref{eq:QCQP.bin}). It can also be the case that the presence of a rank constraint is endogenous to the problem. This is often the case in machine learning, for example, where it is necessary to assume that a solution is low rank, either because the problem is ill-defined without such an assumption or because it reflects some property of the model. Consider e.g. the problem of matrix completion \cite{candes2010matrix}, which is a cornerstone problem in user recommendation systems (see, e.g., the Netflix prize). In this problem, we have access to a matrix $Z \in \mathbb{R}^{m \times n}$, which is partially complete, i.e., some of its entries are specified but others are unknown. The goal is to fill in the unknown entries. Without assuming some structure on $Z$, any completion of $Z$ would be a valid guess and so the problem is ill-defined. This can be remedied by assuming that $Z$ should have low rank. In the context of user recommender systems, this assumption is actually quite natural. Indeed, if one assumes that the matrix $Z$ reflects the ratings a user $i$ ($i=1,\ldots,n$) gives a product $j$ ($j=1,\ldots,m$), then completing the matrix $Z$ would involve infering how a user would have rated a product from existing ratings. Under the assumption that a consumer base can be segmented into $k$ categories (which is a common assumption in marketing), it would then make sense to constrain the matrix $Z$ to have rank less than or equal $k$, which would reflect this segmentation. The matrix completion problem would then be written
%\begin{equation}\label{eq:matrix.completion}
%\begin{aligned}
%&\min_{X \in \mathbb{R}^{m \times n}} &&\sum_{i,j} (X_{ij}-Z_{ij})^2\\
%&\text{s.t. } &&\mbox{rank}(X) \leq k,
%\end{aligned}
%\end{equation}
%where $Z$ is the partially complete matrix corresponding to past data. Similar examples that arise in machine learning include clustering and maximum variance unfolding \cite{kulis2007fast}.

%
%
%[*Something about the algorithms we are going to present are tailored to exactly problems of the form (2). They are NP-hard to solve so some research interest has gone into providing good relaxations for them (nuclear norm etc). This is not what we're doing here. Here, $k$ is very much a parameter of the problem. It is worth mentioning that ]
%
%
%Note that neither (\ref{eq:SDP.rank1}) nor (\ref{eq:matrix.completion}) are SDPs; in fact, they are NP-hard to solve. To obtain SDPs, one needs to relax the initial problems by either dropping the rank constraint (typically, for problems such as (\ref{eq:SDP.rank1})), or by replacing the rank constraint on the matrix by a constraint on its nuclear norm \cite{recht2010guaranteed}. For example, in the case of (\ref{eq:matrix.completion}), the problem could be relaxed to
%\begin{equation}\label{eq:matrix.completion.relaxation}
%\begin{aligned}
%&\min_{X \in \mathbb{R}^{m \times n}, W_1 \in \mathbb{R}^{m \times m}, W_2 \in \mathbb{R}^{n \times n}} \sum_{i,j} (X_{ij}-Z_{ij})^2\\
%&\text{s.t. } \mbox{Tr}\begin{bmatrix} W_1 & X\\ X^T & W_2 \end{bmatrix} \leq k, \begin{bmatrix} W_1 & X\\ X^T & W_2 \end{bmatrix}  \succeq 0.
%\end{aligned}
%\end{equation}
%[*Say something about the two methods here* Burer Monteiro doesn't require dropping the rank constraint as it is hard-coded into the problem as we see next.*]

\subsection{The Burer-Monteiro factorization} \label{subsec:BM}
The key idea of the Burer-Monteiro algorithm \cite{burer2003nonlinear} is to factor the decision variable $X$ as $VV^T$ where $V \in \mathbb{R}^{n \times k}$ (as $k$ is known). The rank-constrained SDP (\ref{eq:rank.SDP}) can then be rewritten equivalently as
\begin{equation}\label{eq:BM}
\begin{aligned}
&\min_{V \in \mathbb{R}^{n \times k}} &&\mbox{Tr}(CVV^T)\\
&\text{s.t. } &&\mbox{Tr}(A_iVV^T)=b_i, i=1,\ldots,m.
\end{aligned}
\end{equation}
As mentioned before, this reformulation has both pros and cons: on the upside, the problem to consider has smaller dimension than (\ref{eq:SDP}) and has no conic constraint to contend with; on the downside, the problem becomes nonconvex. Hence, local optimization methods may not always recover the global minimum of (\ref{eq:SDP}). Research in this area has consequently sought to find an algorithm to solve (\ref{eq:BM}) that (i) provably recovers global solutions to the problem; (ii) does so reasonably fast both in terms of convergence rates and experimentally; and (iii) works on a large class of inputs $A_i, b_i,$ and $C$. We review existing algorithms through the lense of these criteria.

\subsubsection{Augmented Lagrangian Methods}
The method recommended by Burer and Monteiro themselves to solve (\ref{eq:BM}) is a method based on an augmented Lagrangian procedure \cite{burer2003nonlinear},  a quick presentation of which is given in Section \ref{subsec:Aug.Lag.Method} of this paper. The idea is to rewrite (\ref{eq:BM}) as an unconstrained optimization problem by adding terms to the objective that penalize infeasible points. This is done by constructing an augmented Lagrangian function, given here by
$$L_{y,\sigma}(V)=\mbox{Tr}(CVV^T)-\sum_{i=1}^m y_i (\mbox{Tr}(A_iVV^T)-b_i)+\frac{\sigma}{2} \sum_{i=1}^m (\mbox{Tr}(A_iVV^T)-b_i)^2.$$
If $y$ and $\sigma$ are fixed appropriately, then minimizing $L_{y,\sigma}(\cdot)$ will yield an optimal solution. To obtain an appropriate pair $(y,\sigma)$, the following iterative procedure is given: fix $(y,\sigma)$ and minimize $L_{y,\sigma}(\cdot)$ to obtain $V$, then construct a new $(y,\sigma)$ from $V$, and repeat; see Section \ref{subsec:Aug.Lag.Method} for the exact construction. Note that this procedure involves the minimization of $L_{y,\sigma}$ with respect to $V$: choosing an appropriate algorithm to do so is also an important step in the method. The authors in \cite{burer2003nonlinear} suggest using a limited-memory BFGS (LM-BFGS) algorithm to do so. The LM-BFGS algorithm is a quasi-Newton algorithm for unconstrained optimization problems, where the objective is differentiable. Unlike Newton methods, it does not require computing the Hessian of the objective function, constructing instead an approximate representation of it from past gradients. Given that gradients of $L_{y,\sigma}$ can be computed quite quickly under some conditions (see \cite{burer2003nonlinear} for more details), this is a reasonably efficient algorithm to use. One can replace the LM-BFGS subroutine with a subgradient approach if (\ref{eq:rank.SDP}) has additional constraints that are non-differentiable. Furthermore, the augmented Lagrangian approach can be extended to rank-constrained SDPs with inequality constraints of the type $\mbox{Tr}(A_iX) \leq b_i$; see \cite{kulis2007fast}. Though there are no theoretical guarantees regarding convergence, nor speed of convergence, to global solutions, the authors of \cite{burer2003nonlinear} experimentally observe that the algorithm tends to return global minima, doing so in a much smaller amount of time than interior point or bundle methods. The follow-up paper \cite{burer2005local} to \cite{burer2003nonlinear} slightly modifies the augmented Lagrangian function and shows convergence of the algorithm to a global minimum if each minimization of the modified $L_{y,\sigma}(\cdot)$ gives rise to a local minimum, something that is hard to test in practice.

\subsubsection{Riemannian optimization methods}\label{subsubsec:Riemann}
Riemannian optimization concerns itself with the optimization of a smooth objective function over a smooth Riemannian manifold. We remind the reader that a manifold is a space that ``looks linear'' locally and a \emph{Riemannian} manifold $\mathcal{M}$ is a manifold that can be linearized at each point $x \in \mathcal{M}$ by a tangent space $T_x \mathcal{M}$, which is equipped with a Riemannian metric. We say that a Riemannian manifold is \emph{smooth} if the Riemannian metric varies smoothly as the point $x$ varies; see e.g. \cite[Appendix A]{boumal2011rtrmc} for a short introduction to such concepts.  In the Riemannian setting, one can define notions of both gradients and Hessians for manifolds, again, see \cite[Appendix A]{boumal2011rtrmc} for the exact definitions. Using these notions, one can extend the concepts of first-order and second-order necessary conditions of optimality to optimization over manifolds. These are identical to the ones for unconstrained optimization over $\mathbb{R}^n$, except that they involve the analogs of gradient and Hessians for manifolds. Similarly, one can generalize many classical algorithms for nonlinear unconstrained optimization (such as, e.g., trust-region and gradient-descent methods) to the manifold setting. We refer the reader to \cite{absil2007trust,absil2009optimization} for more information on the specifics of these algorithms which we will not cover here.

Though it may not be immediately apparent as to why, Riemannian optimization methods have become a popular tool for tackling problems of the form (\ref{eq:BM}) \cite{journee2010low,boumal2016non}. Indeed,
$$\mathcal{M}=\{V \in \mathbb{R}^{n \times k}~|~\mbox{Tr}(A_iVV^T)=b_i, i=1,\ldots,m\}$$
is a smooth Riemannian manifold under certain conditions on $A_i$ (see \cite[Assumption 1]{boumal2018deterministic}) and the objective function $V \mapsto \mbox{Tr}(CVV^T)$ is also smooth. Hence, (\ref{eq:BM}) is exactly a Riemannian optimization problem. It can be shown that if the conditions on $\mathcal{M}$ that make it smooth hold, and $\mathcal{M}$ is compact, then for almost all $C \in S_n$, any second-order critical point of the problem is globally optimal \cite[Theorem 2]{boumal2016non}. (We use the manifold definition of a second-order critical point here.) If an algorithm which returns second-order critical points can be exhibited, then, in effect, we will have found a way of solving (\ref{eq:BM}). Among all optimization methods defined over Riemannian manifolds, it so happens that the Riemannian trust-region method returns a second-order critical point---under some conditions---regardless of initialization \cite{boumal2018global}. In fact, it is shown in \cite{boumal2018global} that an $\epsilon$-accurate solution (i.e., a solution $V \in \mathcal{M}$ to (\ref{eq:BM}) with $||\mbox{grad}(\mbox{Tr}(CVV^T))|| \leq \epsilon$ and $\mbox{Hessian}(\mbox{Tr}(CVV^T)) \succeq -\epsilon I$ ) can be obtained in $O(1/\epsilon^2)$ iterations. This makes it a popular algorithm to use among all possible algorithms one could use to solve (\ref{eq:BM}) (Riemannian or otherwise) as it has good theoretical guarantees. Other Riemannian methods which come with some theoretical guarantees are the Riemannian steepest-descent algorithm and the Riemannian conjugate gradient algorithm, both of them being known to converge to a critical point \cite{boumal2018global, sato2015new}. In practice though, many more algorithms for nonlinear optimization can be and have been generalized to manifolds (though their convergence properties have not necessarily been studied) and are used to solve problems such as these (see, e.g., the list of solvers implemented in MANOPT, one of the main toolboxes for optimization over manifolds \cite{manopt}). 

We conclude this section by mentioning a few applications where Riemannian optimization methods have recently been used. These include machine learning problems such as synchronization \cite{mei2017solving}, phase recovery \cite{sun2018geometric}, dictionary learning \cite{sun2016complete}, and matrix completion \cite{boumal2011rtrmc}; but also robotics problems such as the \emph{Simultaneous Localization and Mapping (SLAM)} problem. SLAM \cite{probabilistic robotics} refers to the problem of simultaneously estimating the location (or trajectory of locations) of a robot and a model of the robot's environment. Two important versions of the SLAM problem are (i) Landmark SLAM, and (ii) Pose-graph SLAM. The Landmark SLAM problem involves simultaneously estimating the position and orientation of the robot and the location of landmarks in the environment. The Pose-graph SLAM problem is a more restricted version that only requires estimating the position and orientation of the robot at each time-step. Traditionally, these problems have been posed as maximum likelihood estimation (MLE) problems and tackled using general nonlinear optimization methods (which do not come with guarantees on finding globally optimal solutions). % \cite{8-14-15-16-ram}. 
More recently, researchers have proposed semidefinite programming relaxations for the MLE problem arising from SLAM \cite{sesync, 25-27-sesync, 4-6-7-ram}. These relaxations provide exact solutions to the MLE problem assuming that noise in the measurements made by the robot are below a certain threshold (see \cite{se-sync} for exact conditions). In \cite{se-sync}, the authors demonstrate that the resulting SDP admits low-rank solutions and use a Burer Monteiro factorization combined with Riemannian optimization techniques (e.g., a Riemannian trust-region approach)  to solve the SDP. Thus, assuming that the conditions on the measurement noise are satisfied, one can find globally optimal solutions to the MLE problems arising from Pose-graph SLAM (and other related MLE problems arising from camera motion estimation and sensor network localization problems) via this method.

\subsubsection{Coordinate descent methods}

One of the more recent trends for solving problems of the form (\ref{eq:BM}) has been to use coordinate descent (or block-coordinate descent) methods \cite{erdogdu2018convergence,wang2017mixing}. They come with the caveat that they can only be used to solve diagonally-constrained problems, i.e., problems of the type
\begin{equation}\label{eq:diag.constr}
\begin{aligned}
&\min_{V \in \mathbb{R}^{n \times k}} &&\mbox{Tr}(CVV^T)\\
&\text{s.t. } &&||v_i||_2=b_i, i=1,\ldots,m.
\end{aligned}
\end{equation}
where $||\cdot||_2$ is the 2-norm and $v_i$ is the $i^{th}$ row of $V$. Coordinate-descent methods are iterative and very easy to explain for this case \cite{wang2017mixing}. We assume that $b_i=1$ for $i=1,\ldots,m$ for clarity of exposition. Initialization consists in randomly choosing $v_i, i=1,\ldots,n$ on the sphere. Then, at each iteration, an index $i$ is picked and the goal is to find a vector $v_i$ such that $\mbox{Tr}(CVV^T)=\sum_{i,j=1}^n c_{ij}v_iv_j^T$ is minimum. As $||v_i||=1$, it follows that we can replace $c_{ii}$ by $0$ without changing the optimal solution. The problem then is equivalent to minimizing $v_i^T(\sum_{j=1}^n c_{ij}v_j)$ for $||v_i||=1$ and admits a closed form solution:
$$v_i=-\frac{\sum_{j=1}^n c_{ij}v_j}{||\sum_{j=1}^n c_{ij}v_j||}.$$
We update the objective by replacing the previous $v_i$ by this new $v_i$ and proceed to the next iteration. This algorithm can be slightly modified to consider descent on blocks of coordinates, rather than one single coordinate at each time-step \cite{erdogdu2018convergence}. In that setting, it can be shown that if the indexes are picked in a correct way, then coordinate block-descent methods converge to an $\epsilon$-accurate critical point in time $O(\frac{1}{\epsilon})$. Each iteration of coordinate descent methods is much less costly (by an order of $n$ approximately)  than its Riemannian trust region counterpart however. As a consequence, numerical results tend to show that as $n$ increases, using coordinate descent methods can be preferable \cite{erdogdu2018convergence}.

\subsubsection{Other methods} The methods presented above are methods that apply to large classes of problems. Note that many other methods have been developed to cater to more problem-specific formulations (e.g., unconstrained low-rank SDPs); see for example \cite{park2016provable,bhojanapalli2016dropping}.

\subsection{Frank-Wolfe based methods} \label{subsec:FW}

We start this subsection by a quick presentation of the Frank-Wolfe algorithm (also known as the conditional gradient algorithm), a version of which will be used in the algorithms we present. The Frank-Wolfe algorithm was first described in a seminal paper by Frank and Wolfe in 1956. It is an iterative algorithm for constrained optimization problems of the type $\min_{x \in S} f(x)$, where $S$ is compact and convex and $f$ is convex and differentiable. At each step $k$, a linear approximation of $f$ (obtained by taking the first-order Taylor approximation of $f$ around the current iterate $x_k$) is minimized over $S$ and a minimizer $s_k$ is obtained. The next iterate $x_{k+1}$ is then constructed by taking a convex combination of the previous iterate $x_k$ and the minimizer $s_k$ before repeating the process. Intuitively, the reason why Frank Wolfe algorithms are popular for rank-constrained SDPs is due to the following fact: if the algorithm is initialized with a rank-1 matrix and if each minimizer is also a rank-1 matrix, then the $k^{th}$ iterate is of rank at most $k$. This enables us to control the rank of the solution that is given as output. We first present an algorithm developed by Hazan \cite{hazan2008sparse} before [****to complete****]
[***CHECK MINIMUM/MAXIMUM and PLUS/MINUSES IN HAZAN ALGORITHM AND MADELEINE. USE SLIDES OF FREUND TO DO THIS***]

\subsubsection{Hazan's algorithm}
Hazan's algorithm is an algorithm which is designed to produce low-rank solutions to SDPs of the type
\begin{equation}\label{eq:SDP.compact}
\begin{aligned}
&\min_{X \in S_n} &&\mbox{Tr}(CX)\\
&\text{s.t. } &&\mbox{Tr}(A_iX)=b_i,~i=1,\ldots,m\\
& &&X \succeq 0 \text{ and } \mbox{Tr}(X)=1.
\end{aligned}
\end{equation}
Note the presence of the additional constraint $\mbox{Tr}(X)=1$, which restricts the applicability of this method. The constraint on the trace can be slightly relaxed to $\mbox{Tr}(X)\leq t$, where $t$ is fixed \cite[Chapter 5]{gartner2012approximation}, but we will consider the case $\mbox{Tr}(X)=1$ here. A key subroutine of the algorithm is solving the following optimization problem:
\begin{equation}\label{eq:Hazan}
\begin{aligned}
&\min_{X \in S_n} &&f(X)\\
&\text{s.t. } &&\mbox{Tr}(X)=1 \text{ and } X\succeq 0,
\end{aligned}
\end{equation}
where $f$ is a convex function. Let $f^*$ be the optimal value of this problem. It is for this subroutine that a Frank-Wolfe type iterative algorithm is used. It can be described as follows: initalize $X_1$ to be a rank $1$ matrix with trace one. Then, at iteration $k$, compute the eigenvector $v_k$ corresponding to the minimum eigenvalue of $\nabla f(X_k)$. Finally, for a fixed parameter $\alpha_k$, set $X_{k+1}=(1-\alpha_k)X_k+\alpha_k v_kv_k^T$ and reiterate. This algorithm returns a $\frac{1}{k}$-approximate solution (i.e., a matrix $X$ such that $\mbox{Tr}(X) \leq 1+\frac{1}{k}$ and $f(X) \leq f^*+\Omega(\frac{1}{k})$) with rank at most $k$ in $k$ iterations. This is of interest in itself as some problems can be cast in the form (\ref{eq:Hazan}), an example being given in \cite{hazan2008sparse}.

It can also be used, as mentioned previously, to solve (\ref{eq:SDP.compact}). To see how this is done, first note that one can reduce solving (\ref{eq:SDP.compact}) to solving a sequence of SDP feasibility problems via the use of bisection. It is enough as a consequence to explain how one can leverage the Frank-Wolfe type algorithm described above to solve an SDP feasibility problem of the type: $\mbox{Tr}(A_iX) \leq b_i,i=1,\ldots,m, X\succeq 0, \mbox{Tr}(X)=1$. Quite straightforwardly, this can be done by letting $f(X)=\frac{1}{M} \log(\sum_{i=1}^m e^{M\cdot (\mbox{Tr}(A_iX)-b_i)})$ where $M=k\log(m)$, $\frac{1}{k}$ being the desired accuracy; see \cite{hazan2008sparse}. The algorithm is then guaranteed to return a $\frac{1}{k}$-approximate solution of rank at most $k$ in $O(k^2)$ iterations.

It is interesting to note that this latter algorithm is nearly identical to the Multiplicative Weights algorithm for SDPs which also produces low-rank solutions \cite{arora2012multiplicative} and has exactly the same guarantees. However it is derived in a completely different fashion.

\subsubsection{Other methods based on Frank-Wolfe}
A caveat of Hazan's algorithm is that the rank of the solution returned is linked to its accuracy. One could maybe think that, as the solution is known to be low-rank and the Frank-Wolfe algorithm is initialized with a low-rank matrix, then all iterates of the algorithm would be low-rank. Unfortunately this is not the case. In fact, what can be observed in practice is that the Frank-Wolfe algorithm typically returns iterates with increasing rank up to a certain point, where the rank decreases again, with the final solution returned being low-rank; see, e.g., the numerical experiments in \cite{yurtsever}. As a consequence, if one requires an accurate solution, one will likely have to deal with high-rank intermediate iterates, with the storage and computational problems that this entails.

In this section, we present two different methods designed to avoid these issues. To the best of our knowledge, these methods only apply to a specific class of optimization problems of the type:
\begin{equation}
\begin{aligned}
&\min_{X \in \mathbb{R}^{n \times d}} f(\mathcal{A}Z)\\
&\text{s.t. } ||X||_{N}\leq 1,
\end{aligned}
\end{equation}
where $f$ is a convex and differentiable function, $||\cdot||_N$ is the nuclear norm of the matrix $X$ \cite{BenMaryamPabloRank}, and $\mathcal{A}:\mathbb{R}^{n\times d} \rightarrow \mathbb{R}^m$ is a linear operator, mapping $X$ to $[\mbox{Tr}(A_1X),\ldots,\mbox{Tr}(A_mX)]$. Note that e.g. the problem of matrix completion described in Section \ref{subsec:apps.low.rank} can be relaxed to a problem of this type. The Frank-Wolfe algorithm can be applied to problems of this type quite readily. Initialization is done as before by setting $X_0$ to be some rank-1 matrix. At iteration $k$, one computes an update direction by finding a pair $(u_k,v_k)$ of singular vectors corresponding to the maximum singular value of $
\mathcal{A}^*( \nabla f(\mathcal{A}X_k))$ where $\mathcal{A}^*:\mathbb{R}^m \mapsto \mathbb{R}^{n \times d}$ is the dual linear operator to $\mathcal{A}$ given by $\mathcal{A}^*z=\sum_{i=1}^m z_i A_i$. We then construct a new iterate $X_{k+1}=(1-\alpha)X_k-\alpha u_kv_k^T$ and repeat.

[**Rewrite this this is the gist***]

The first method, described in \cite{Freund}, is a modification of the previously defined algorithm. The key idea is that at every iteration, the algorithm chooses between two types of steps. One type is the previously mentioned step (called the ``regular'' step in the paper); the other is what is called an ``in-face step''. Quite simply, instead of optimizing **to finish instead of optimizing the gradient thingey over the whole of the nuclear norm ball, it is instead optimized over the minimum size face to which the current iterate belongs (or an away step is used there are two different ways of doing this). This means that the rank of the next iterate is that of the current one, it can actually be even less if we go all the way to the boundary of the face. The advantage of working with the faces of the nuclear norm unit ball is that we know what the faces look like and we can optimize over them in an efficient manner. This is what makes a generalization to other types of problems complicated. Under some conditions on how to choose which step, after $k$ iterations, we still have a $\frac{1}{k}$-approximate solution. The rank however can be less than $k$ depending on the amount of ``in face'' steps used and more importantly one can avoid ever dealing with high-rank intermediate iterates if enough of these in-face steps are used.

The second method described in \cite{yurtsever} focuses on the storage issues generated by dealing with the high-rank intermediate iterates. Never stores the intermediate high-rank iterates.
